Inducing Gaussian Process Networks

Gaussian processes (GPs) are powerful but computationally expensive machine learning models, requiring an estimate of the kernel covariance matrix for every prediction. In large and complex domains, such as graphs, sets, or images, the choice of suitable kernel can also be non-trivial to determine, providing an additional obstacle to the learning task. Over the last decade, these challenges have resulted in significant advances being made in terms of scalability and expressivity, exemplified by, e.g., the use of inducing points and neural network kernel approximations. In this paper, we propose inducing Gaussian process networks (IGN), a simple framework for simultaneously learning the feature space as well as the inducing points. The inducing points, in particular, are learned directly in the feature space, enabling a seamless representation of complex structured domains while also facilitating scalable gradient-based learning methods. We consider both regression and (binary) classification tasks and report on experimental results for real-world data sets showing that IGNs provide significant advances over state-of-the-art methods. We also demonstrate how IGNs can be used to effectively model complex domains using neural network architectures.

==> data/reviews_50.tex <==
\begin{enumerate}
\item \textbf{positive} - there have been several films about zorro some even made in europe e g alain delon this role has also been played by outstanding actors such as tyrone power and anthony hopkins but to me the best of all times has always been reed hadley this serial gives you the  ...  of various actors of movies b like ed cobb ex tarzan jim pierce c shaw eternal villains like john and charles king and a very good performance of hadley as zorro he was quick smart used well his whip and sword and his voice was the best for any zorro
\item \textbf{negative} - i love the frequently masters of horror series horror fans live in a constant lack of projects like this and the similar project with gave us feast like it or lump it are breeding grounds for wonderful thought bubbles in the minds of directors with a horror bent to develop  ...  get it but well the worst curse of storytelling a rousing and promising set up without a rewarding denouement br br cue to your build up has to have a payoff that exceeds build up not the other way around storytelling math 101 br br end of spoilers big oops
\item \textbf{positive} - i rented the film i don't think it got a theatrical release here out expecting the worse the previews made the film look awful i was in fact very surprised it was well worth watching it was loosely scripted almost like an ensemble piece of film it had some very  ...  it is the fashion to be critical of jerry springer he is also an easy target springer could have made citizen kane and it would be proclaimed 'the worst film ever i recommend this film for anybody interested in the show a flawed but innovative and interesting piece of film
\item \textbf{positive} - one of the best of the fred astaire and rogers films great music by irving berlin solid support from randolph scott harriet nelson lucille ball betty grable frank and br br terrific songs include let yourself go let's face the music and putting all my eggs in one basket the  ...  has the bigger role but is only ok br br rogers has one of her best solo numbers in the series with let yourself go jazzy and it's a great song br br fun all the way although i got tired of we joined the navy after the third time
\item \textbf{positive} - forbidden planet rates as landmark in science fiction carefully staying within hard aspects of the genre science not fantasy nerds will love it while still playing with imagery and ideas of contemporary 1950s values isolated house is a model of modern design with open spaces that step out into gardens  ...  away from her father her home to leave with the sailors for earth it's this act of defiance of maturity that sends id creature over the edge destroying its creator just as it did thousands of centuries earlier to the krell br br maybe the krell had teenage daughters too
\item \textbf{negative} - the bad news is it's still really dreadful i gave it a 2 because occasionally some of this slapstick parody actually seems funny br br it's supposed to be better than zombie ass kicker and progress should be rewarded or maybe i was drinking heavily when i watched it and  ...  mess into about an hour of truly awful amateur video br br you'd best smoke a lot of something powerful if you want to enjoy this one and get this dvd back to the video store on time you'll really hate yourself if you have to pay a late fee
\item \textbf{positive} - nice character development in a pretty cool milieu being a male i'm probably not qualified to totally understand it but they do a nice job of establishing the restrictive victorian environment from the start it isn't as bleak as it really was and the treatment of women was probably even  ...  human beings who get to see the light i did have a little trouble with the alfred molina character having such an epiphany so quickly but within this world it needed to happen good acting all around with something positive taking place in the lives of some pretty good people
\item \textbf{negative} - mercifully there's no video of this wannabe western that a stay afloat vehicle for big frank at a time when his career was floundering the story of a who lives on the reputation of his big gun brother and who gets run out of town by bad guys only to  ...  reviewer who found it underrated the critics slammed it at the time and deservedly so you'll have to catch it on the last show if you up late and having a bout of insomnia but if you can sit through it you've more than most of my movie buff friends
\item \textbf{negative} - bela lugosi is an evil who sends brides poisoned on their wedding day steals the body in his fake ambulance hearse and takes it home for his midget assistant to extract the in order to keep wife eternally young some second rate actors playing detectives try to solve the terrible  ...  ridiculous tell anyone what happens in it and they tend to laugh quite a lot and demand to see the film i got the dvd in a discount store 2 for £1 which i think is a pretty accurate anyone paying more for this would be out of their mind
\item \textbf{positive} - its no surprise that busey later developed a in his this film is also a poor decision but one i enjoyed fully the first 5 minutes is the most uninspiring 5 minutes in any film boring bad and then with a spiderman stance busey yells the best worst line in  ...  physics and absurdity and lastly when mcbain jumps out of the during intense guerrilla warfare and starts to run and a small object i almost wet myself some of best work by far rent or buy it today my vote is a perfect 10 on the poo meter that is
\item \textbf{positive} - before sky i saw diane tender performance in this otherwise of a movie campers are invited to the camp of their youth and experience it as adults each of those that return seem to be looking for something they lost which makes it so realistic maybe you had to be  ...  paxton diane elizabeth mrs brad probably when he first fell for her the beautiful scenery bright colors comical music including variations of hello and a comic acting turn by noted director sam raimi makes this a movie you can pull out again and again like looking up an old friend
\item \textbf{positive} - the line of course is from the lord's prayer thy will be done on earth as it is in heaven sweden especially its far north is not my idea of heaven 30 degree c winter are a little on the low side for me but the good folk who live  ...  nyqvist is simply wonderful as daniel the frail but driven musician and there's some nice music as well i was for the whole two hours the ending is what you make of it i guess but it's not spoiling it to say daniel achieves what he set out to do
\item \textbf{positive} - my certainly is a fair looking woman this film is a lost gem a dead on satire mockumentary of the early 90's hip hop scene when mc hammer had just began to fade away into that good night we follow the three members of the as they embark upon their  ...  films that no one has ever heard of but it's the kind of film you either love or hate a lot like company man in this regard i regard this movie like the 1000 islands of upstate new york it's a wonderful little secret you want to keep to yourself
\item \textbf{positive} - i rented this film from netflix for two reasons i was in the mood for what i thought would be a silly '50s sci fi and because it is the first feature length superman film needless to say after about 15 minutes i found myself thoroughly engaged and very pleasantly  ...  by today's standards the costuming is poor to fair but for its time this film's special effects and costuming were quite good the cinematography is also generally very good and the acting is much better than one might expect i was particularly impressed with reeves jeff corey and walter reed
\item \textbf{negative} - brilliant book with wonderful characterizations and insights into human nature particularly the nature of addiction which still resonate strongly today br br as for the movie eh nothing special the cameraman clearly had an unfortunate addiction to circling and circling and circling around everything making the viewer quite nauseous why  ...  didn't put a stop to this is beyond me but maybe he was too busy trying and somehow failing to draw good performances from these normally excellent but inappropriately cast actors all in all a weak adaptation your three hours would be better spent reading or re reading the book
\item \textbf{negative} - it's boggles the mind how this movie was nominated for seven oscars and won one not because it's abysmal or because given the collective credentials of the creative team behind it really ought to deserve them but because in every category it was nominated honor disappoints some would argue that  ...  in the early 70's and huston's direction is as uninteresting as everything else there's promise behind the story and perhaps in the hands of a director hungry to be recognized it could've been morphed to something better but what's left looks like a film nobody was really interested in making
\item \textbf{positive} - a comedy of funny proportions from the guys that brought you south park and most of the guys from this movie has utterly disgusting and satirical content it portrays incredibly cruel treatment of humans and animals i love it this is some funny stuff really funny two loser friends create  ...  is some funny stuff really funny two loser friends create a game in driveway which explodes into a national sensation corruption and greed and blackmail turn the sport sour and its up ta coop ta fix it and along the way you will laugh alot that's all there is enjoy
\item \textbf{negative} - there was a bugs bunny cartoon titled baby buggy bunny that was exactly this plot baby faced robbed a bank and the money in the carriage rolled away and fell into bug's rabbit hole he dressed up as a baby to get into hole to retrieve the money the scene  ...  straight from the cartoon this was a hilarious 5 minute cartoon not so much an entire movie if you are really interested in this buy the bugs bunny dvd it's was much more original the first time 1954 plus you'll get a lot more classic bugs bunny cartoons to boot
\item \textbf{negative} - first off i really loved henry fool which puts me in a very small pool of movie goers parker posey is one of best actresses on screen today but this film was a full out travesty watching hartley and the actors talk about the film in the extras so full  ...  a smile br br when i saw the trailer i thought oh they're just trying to grab a new audience but it's really this ridiculous ride i'd be happy to spoil this movie for you but it's been done it's rotten the fool franchise is dead long live henry fool
\item \textbf{positive} - i imagine victorian literature slowly sinking into the of the increasingly distant past pulled down by the weight of its under skirts along comes television at its best it has a power and with like those the bbc produce so finely victorian literature gets a new stab at life the  ...  that you're almost with him at the end no one's perfect the supporting cast ably create a world into which you sink without feeling that coarse have been made to modern tastes and without having felt preached to another bbc classic highly recommended this is how romantic literature should be
\item \textbf{negative} - i knew this movie wasn't going to be amazing but i thought i would give it a chance i am a fan of luke wilson so i thought it had potential unfortunately a lot of the movie's dialog was very fake sounding and cheesy i think that gave some money  ...  you can't help but notice it maybe they should have focused on writing and acting more than how many times can we drop products in the movie without people getting annoyed the movie had its moments but i'm glad i didn't spend 9 50 to see it in the theater
\item \textbf{negative} - i have read several good reviews that have defended and the various aspects of this film one thing i see over and over is annoyance with megan the idealistic political scientist trying to change the world i loved her character maybe because i am a 23 year old political science  ...  probably the best character br br i give this film 4 out of 10 it had a good setting almost no plot and a mix of good and terrible acting i would recommend it for a cheap thrill but hardly a diamond in the rough that is micro budget horror
\item \textbf{negative} - this movie is like the thousand cat and mouse movies that preceded it the following may look like a spoiler but it really just describes a large class of movies there is the passionate wise main character his goofy but well meaning sidekick with his ill placed attempts at humorous  ...  easily predicted and i can assure you i am not the tool in the shed i am quite tired of feeling tricked for money after exiting the theater from a hollywood movie and if you have ever felt that way too heed my warning stay miles away from this movie
\item \textbf{negative} - i wonder who how and more importantly why the decision to call richard attenborough to direct the most singular sensation to hit broadway in many many years he's an academy award winning director yes he won for you moron jeremy irons is an academy winning actor do you want to  ...  been cast with stars unknown newcomers but stars with compelling unforgettable faces even the most invisible of the group great actors who could dance beautifully well michael douglas was in it true i forgot i'm absolutely wrong and you are absolutely right nothing like a richard attenborough michael douglas musical
\item \textbf{positive} - this movie will go down down in history as one of the greats right along side of citizen kane casablanca and on the waterfront someone please convince leno to do a sequel leno and morita are a comedy duo the likes of which haven't been seen since abbot and costello  ...  it for you but it makes the explosion of the death star pale in comparison if you can track down this hard to find gem do yourself and your family a favor and buy it immediately i'm still holding out hope for a special edition dvd one of these days
\item \textbf{negative} - this is high grade cheese fare of b movie kung fu flicks bruce wannabe lee is played by bruce li i think of course let's show quick clips of bruce and do closeups of his eyes and if you at the right angle during a certain time of the day  ...  kay bee you see bruce also finds nothing wrong with savagely beating up a crippled man towards the end the director decided let's throw a flashback for a scene just shown 3 minutes ago they must've thought that only one with attention disorder could fully understand this film br br
\item \textbf{negative} - the only previous gordon film i had watched was the kiddie adventure the magic sword 1962 though i followed this soon after with empire of the ants 1977 he seems to be best remembered however for his sci fi work of the 1950s br br anyway i happened upon this  ...  scenes do stick out the hilarious opening ceremony and other would be erotic the overall quality of the film would have still been poor without them then again this particular version is further sunk by the tacked on electronic score – which is wholly inappropriate and cheesy in the extreme
\item \textbf{positive} - hilarious evocative confusing brilliant film reminds me of or holy mountain lots of strange characters about and looking for what is it i laughed almost the whole way through all the while keeping a peripheral eye on the bewildered and occasionally horrified reactions of the audience that surrounded me in  ...  is it than 5000 movies like titanic or sleepless in seattle shudder gag groan br br thank you mr glover additionally a fun man to watch on screen or at his big slide show smart funny quirky and outrageously hot make more films write more books keep the nightmare alive
\item \textbf{positive} - the villian in this movie is one mean sob and he seems to enjoy what he is doing that is what i guess makes him so mean i don't think most men will like this movie especially if they ever cheated on their wife this is one of those movies  ...  the ending we would like to see but not the ending to such a mean beginning and then there is the aftermath of what happened guess you can make up your own mind about the true ending i'm left feeling that only one character should have survived at the end
\item \textbf{negative} - okay what the hell kind of trash have i been watching now the mountain has got to be one of the most incoherent and insane spanish exploitation flicks ever and yet at the same time it's also strangely compelling there's absolutely nothing that makes sense here and i even doubt  ...  mountain is occasionally very creepy with its spooky music and interesting cinematography the supportive characters all look uncanny and the ravishing patty shepard plays a good heroine this is the type of european horror film that could have been legendary if only someone had bothered to write a structured screenplay
\item \textbf{positive} - i found this movie to be very good in all areas the acting was brilliant from all characters especially ms stone and character just gets smarter and more psychologically twisted by the minute the plot is interesting even though this movie is more for the mind playing between the main  ...  whole atmosphere of the movie was that mysterious thriller like masterpiece go see this film now it deserves better than what it got from the audience which was misled by some faulty terrible reviews about the movie before it even started you won't regret it if you go see it
\item \textbf{negative} - a lot of horror fans seem to love scarecrows so i won't be very popular in saying that i found it to be rather boring the idea behind it was interesting but it seems to drag so much i think the main problem is that it is all set in  ...  most were hard to even see if a little more lighting had been used perhaps it could've been better br br there's not many films involving killer scarecrows to my knowledge apart from dark night of the scarecrow which is much better i would recommend that over scarecrows any day
\item \textbf{negative} - david mamet's film debut has been hailed by many as a real thinking man's movie a movie that makes you question everybody and everything i saw it for the first time recently and couldn't understand what was supposed to be so great about it br br the movie is about  ...  not only that but she didn't even take back the money he stole from her br br ultimately the movie leaves you feeling empty and unfulfilled and if you like me predicted ahead of time that margaret was going to be conned you will find this revelation just as unsatisfying
\item \textbf{positive} - while this was a better movie than 101 dalmations live action not animated version i think it still fell a little short of what disney could do it was well filmed the music was more suited to the action and the effects were better done compared to 101 the acting  ...  family film with little or no material and yet it remains fun and interesting for adults and children alike it's bound to be a classic as so many disney films are here's to hoping the third will be even better still because you know they probably want to make one
\item \textbf{positive} - i think i read this someplace joe johnston director of the film and also one of the guys who founded industrial light and magic for work on the first star wars film and one of his producers or something were their brains for a title for the movie rocket boys  ...  is october sky they were shocked to say the least the title summed up everything in the movie since the movie revolves around sputnik at first homer jr did not like the idea but he warmed up to it after the movie poster paperback novel came out and took off
\item \textbf{positive} - stephen king movies are a funny thing with me i either really love them or i loathe them some of the productions such as desperation and storm of the century i didn't enjoy some of the smaller ones i really loved sleepwalkers is one that i really do enjoy and  ...  town with lots of interesting characters the acting isn't the best nor are the special effects however somehow the whole thing tends to and is very watchable and enjoyable adaption br br for uk readers this production has most recently been shown on sci fi and sky thriller horror channels
\item \textbf{positive} - if you're researching ufo facts then this video is very important the of the video is the comments made by buzz he is without a doubt from the best of america trained to be objective honest and factual in his reports many astronauts from america of all eras have reported  ...  does contain further information and opinions from an accomplished american hero those don't come along every day so the fact that some people aren't interested in details should not detour your from viewing this video if nothing else it is interesting and i recommend you watch with an open mind
\item \textbf{positive} - rupert friend gives a performance as prince albert that lifts the young victoria to unexpected levels he is superb as we know queen victoria fell into a dark deep depression after prince albert's death and looking into friend's eyes i understood the film doesn't take us to his death but  ...  i believed what he felt was real nothing or anybody gets anywhere near the and of friend's characterization emily blunt is good but i didn't believe for a minute she was victoria no real sense of period it may no have been her fault but her prince deserved the crown
\item \textbf{positive} - seeing moonstruck after so many years is a reminder of how sweet and funny this film was when it first appeared who knew that cher could act who had ever heard of olympia dukakis nicholas cage was the beginning of his career and vincent gardenia and danny aiello were not  ...  films of this genre in the meantime all the actors acquit themselves admirably and the audience enjoys itself in its way moonstruck is how hollywood used to be at its best entertainment with no social significance whatsoever if they'd only lost that's along the way it would have been perfect
\item \textbf{negative} - i first learned of the wendigo many years ago in one of alvin scary stories books according to that story the wendigo after calling your name in the wind drags you along and then pulls you up into the sky and you while it sounds like a pretty bizarre notion  ...  asking for it and everyone had better listen to the old indian guy i've seen this stuff so many times that i no longer bother to count br br anyway avoid it patricia clarkson and erik per sullivan dewey on malcolm in the middle have done far better than this
\item \textbf{positive} - well maybe not immediately before the rodney king riots but even a few months before was timely enough my parents said that they saw it and the next thing you know the police got and la got burned to the ground it just goes to show the state of race  ...  people's interest in race relations but this one came out much earlier maybe we'll never be able to have stable race relations in this country but either way grand canyon is a great movie it kevin kline as my favorite actor also starring mary mary louise parker and alfre woodard
\item \textbf{positive} - finally a movie where the audience is kept guessing until the end what will happen well we all kind of know that the lives of the brothers andy played by hoffman and hank played by hawke will spiral downward towards destruction since where else is there to go but down  ...  the part well enough add into this mix andy's wife played perfectly by marisa tomei cheating with hank andy's of company funds to pay for his drug and sex addictions and a father who finally discovers exactly what happened the day of the robbery this movie will get you thinking
\item \textbf{negative} - wow i don't even really remember that much about this movie except that it stunk br br the plot's basically a girl's parents neglect her so this pokemon pretends to be her dad am i the only one disturbed by that then this weirdo pokemon kidnaps mom to pretend to  ...  br br that's pretty much all i can remember but i think you can take it as a hint and not see it or if you do see it don't expect much 1 out of 10 br br seriously if you want a pokemon movie rent pokemon the first movie
\item \textbf{positive} - the group of people are travelling to in an awful bus led by a drunk conductor and his dumb son who likes to drive with his eyes closed their journey is frequently interrupted by many hilarious events which with much irony describe the fall of nation s spirit in 1941  ...  as a common jokes the man who steals the show is a peasant 4 feet tall with his 4 sons who are almost two times bigger than him in the end the movie takes one turn and the trip becomes nothing but a swan s song of a dying country
\item \textbf{negative} - yes this movie is a real thief it stole some shiny oscars from just because politicians wanted another war hero movie to boost the acceptance support for the wars u s is still fighting today i do not really want to go here into politics but come on this is  ...  like and what not to like the same propaganda movies were produced that time only with the exception that those were black and white even if we consider this title a reasonable piece of the u s wars are cool genre you surely have much better movies to choose from
\item \textbf{positive} - i was going through a list of oscar winners and was surprised to see that this film beat butch cassidy and the sundance kid for best picture in 1969 after actually seeing it however i'm not surprised anymore it was way ahead of its time in regards to its style  ...  to see if it's really him that has done or is about to do something terrible br br i think it was a brilliant decision by hoffman to take this role otherwise he may have been typecast after the graduate anyway this considered an all time great for a reason
\item \textbf{positive} - inspirational tales about triumph of the human spirit are usually big turn offs for me the most surprising thing about men of honor is how much i enjoyed it in spite of myself the movie is as predictable and cliched as it gets but it works much credit goes to  ...  leads it's a perfect role for cuba gooding jr who's wonderfully restrained here we have come to expect a lot from de niro and he doesn't disappoint he creates a darkly funny portrait director george jr set out to make an old style flick and comes up with a winner
\item \textbf{negative} - this movie was god awful from conception to execution the us needs to set up a star wars site in this remote country this is their premise the way to gain access the us concludes is to win an obstacle course like cross country race where the winner can ask  ...  ninjas with machine guns was enough to get me to rent this film br br but if i were ever to meet kurt thomas the gymnast star in real life i would probably kick him in the face after a double with 2 1 2 twists in the layout position
\item \textbf{positive} - i wouldn't call we're back a story simply a kiddie version of jurassic park i found it more interesting than that like the former it calls into question the security of bringing beings from one era into ours but it really opens my eyes when i see who provided the  ...  on the cast i thought that this movie had something for both children purely fun and adults natural history true it's escapism but the perceptive kind i would actually say that john goodman doing voice here is sort of a precursor to his voice work in monsters inc worth seeing
\item \textbf{negative} - chinese ghost story iii is a totally superfluous sequel to two excellent fantasy films the film delivers the spell casting special effects that one can expect but fails painfully on all other fronts the actors all play extremely silly caricatures you have to be still in to find their slapstick  ...  br br it is astonishing to see what trash fantasy fans have to put up with in this case because somebody thought they could squeeze a little extra money out of a successful formula they won't be able to do it again the cash cow is now dead as a
\item \textbf{negative} - the direction had clearly stated that this film's idea and plot is totally original however as to those who have read comic we can clearly see that the characters are very similar and even some jokes br br another note is jay chow himself do not know kung fu it  ...  i think why jay is the main actor is simply is for his popularity br br despite how hard i wish to stop anyone from watching this thus making this movie getting what it shouldn't have it has became one of the best budget films in china for this year
\item \textbf{negative} - let me start by saying that i understand that invasion of the star creatures was meant to be a parody of the sci fi films of the 50s i understand that none of it is to be taken seriously the problem i have is that none of it works a  ...  chase sequences dancing indians men rings and other assorted unfunny bits it's all just a complete waste of time br br i bought this on the double feature dvd with invasion of the bee girls that movie is academy award winning stuff in comparison with invasion of the star creatures
\item \textbf{positive} - knowing when to end a movie is just as important as casting directing and acting and it's nice to see when a director script get it right clocking in at just 82 minutes 10 items or less doesn't stretch the story trying to grasp at inane topics it stays focused  ...  they know when to say goodbye and what each garnered from the other it's a quiet but riveting moment as clunker car sits outside l a mansion br br this is a great independent production and one that wastes little time getting going and it won't waste your time either
\item \textbf{negative} - italian born has inherited from her deceased lover karl an ultra modern and isolated house in the middle of the woods it's winter and she meets the mysterious caretaker leslie who eventually ends up not only just looking after the house but also that of as she tries to adapt  ...  seymour cassel pokes his head in now and then br br just where is it heading is anyone's guess well that's if you can wait around for it i think i'll give it the benefit of the doubt as it's definitely not what i was expecting from this indie film
\item \textbf{negative} - is a horror comedy that doesn't really have enough horror or comedy to qualify as one or the other it has one scene that is exceptionally good any number of that work but very few real scares and not enough humor to maintain the movie in addition the script does  ...  in many ways it was stronger primarily because the main characters were stronger but more importantly because it looked beautiful although that may be preferring the movie that is weaker in general plot and spine because of production values that just shows you how uninteresting i found the look of
\item \textbf{positive} - there were a lot of 50's sci fi movies they were big draws for the drive in theaters a lot of them were crappy even back then this movie and 'the day the earth stood stand out and both have aged well in their own way from the very beginning  ...  was a new movie and it scared me of course every movie that was even vaguely scary did back then but i remember being real worried about the invisible monster forbidden planet is a movie a sci fi fan can watch several times and find something new with each viewing
\item \textbf{negative} - curiously it is rene eyes and mouth not buddy the that emerge as the focal point of buddy a jim henson pictures production through francis ford somehow countless close ups of face slipped passed in the post production stages and she literally fills the screen so many times the poor  ...  furniture should be the least of anyone's worries in this do failure but at least we know russo was in good hands whenever director caroline thompson needs a good pick up shot she gives rene another extreme close up i wonder what the lipstick budget was on this picture from
\item \textbf{positive} - now this is what i'd call a good horror with occult supernatural undertones this nice low budget french movie caught my attention from the very first scene this proves you don't need wild fx or lots of gore to make an effective horror movie br br the plot revolves around  ...  seen there a few flaws though the fx are not that good but they're used effectively the plot leaves some mysteries open and things get very confusing towards the end but redeems itself by the time it's over br br i thought his was a very good movie 8 10
\item \textbf{negative} - and ethel buffs too will love her loud vocals as the wicked witch but this cartoon sequel to the wizard of oz is bereft of real imagination substituting fantasy and excitement with noisy action and cheaply repeating its footage like a bad music video little dorothy is whisked back to  ...  can count on minnelli for energy which is why the movie up whenever dorothy is around much of it is unmemorable and i'm not even sure baby boomers will get a charge from it since it has been out of for so long as a curiosity item just fair from
\item \textbf{negative} - this is another one of those vs insects features a theme that was popular in the late 70's only you can't really call it horror there's zero suspense and no gruesome events in other words this movie is pretty lame it's not that it's really bad or something it's just  ...  movie from 1976 was much better than this one i even feel i have to go back and add a few points to its rating after having seen ants lacking suspense action thrills shocks and creepiness the only thing you'll be left with after seeing ants is an annoying itch
\end{enumerate}
